Accessibility and presentability in 2-categories

We outline a definition of accessible and presentable objects in a 2-category $\mathcal K$ endowed with a "KZ context", that is to say a pair of lax-idempotent monads interacting in a prescribed way; this perspective suggests a unified treatment of many "Gabriel-Ulmer like" theorems, asserting how presentable objects arise as reflections of generating ones. We outline the notion of "(Gabriel-Ulmer) envelope" for a KZ context, sufficient to concoct Gabriel-Ulmer duality. We end the paper with a roundup of examples, involving classical (set-based and enriched), low dimensional category theory, and a perspective for future work, rooted in higher category theory and homotopy theory.

==> layout/L-abstract.tex <==
\begin{abstract}
	We outline a definition of accessible and presentable objects in a 2-category $\cK$ endowed with a ``KZ context'', that is to say a pair of well-interacting lax-idempotent monads; this perspective suggests a unified treatment of many ``Gabriel-Ulmer like'' theorems, asserting how presentable objects arise as reflections of generating ones. We outline the notion of \emph{(Gabriel-Ulmer) envelope} for a KZ context, sufficient to concoct Gabriel-Ulmer duality. We end the paper with a roundup of examples, involving classical (set-based and enriched), low dimensional and a perspective for future work, rooted in higher category theory and homotopy.
\end{abstract}

==> layout/L-title-addr.tex <==
\title{Accessibility and presentability in 2-categories}

\author[1]{Ivan Di Liberti}
\author[2]{Fosco Loregian}

\affiliation[1]{Mondo}
\affiliation[2]{Mondo}

% \begin{minipage}{.475\textwidth}
%   $^\ddag$Institute of Mathematics, \newline
%   Czech Academy of Sciences,\newline
%   Prague, Czech Republic.\newline 
%   Department of Mathematics and Statistics\newline 
% \end{minipage}%
% \begin{minipage}{.475\textwidth}
%   $^\dag$Tallinn University of Technology,\newline
%   Tallinn, Estonia.\newline  
% \end{minipage}
% \address{
%  $^\ddag$Institute of Mathematics, \newline
%   Czech Academy of Sciences,\newline
%   Prague, Czech Republic.\newline 
%   Department of Mathematics and Statistics\newline
%   }
% \url{diliberti.math@gmail.com}
% \address{
%   $^\dag$Tallinn University of Technology,\newline
%   Tallinn, Estonia.\newline
%   }
% \url{fosco.loregian@taltech.ee}

